MetaXL: Meta Representation Transformation for Low-resource Cross-lingual Learning

The combination of multilingual pre-trained representations and cross-lingual transfer learning is one of the most effective methods for building functional NLP systems for low-resource languages. However, for extremely low-resource languages without large-scale monolingual corpora for pre-training or sufficient annotated data for fine-tuning, transfer learning remains an under-studied and challenging task. Moreover, recent work shows that multilingual representations are surprisingly disjoint across languages, bringing additional challenges for transfer onto extremely low-resource languages. In this paper, we propose MetaXL, a meta-learning based framework that learns to transform representations judiciously from auxiliary languages to a target one and brings their representation spaces closer for effective transfer. Extensive experiments on real-world low-resource languages - without access to large-scale monolingual corpora or large amounts of labeled data - for tasks like cross-lingual sentiment analysis and named entity recognition show the effectiveness of our approach. Code for MetaXL is publicly available at github.com/microsoft/MetaXL.

==> tables/main_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
\begin{wraptable}{r}{7.5cm}
\vspace{-4mm}
\begin{tabular}{@{}llll@{}}
\toprule
                        & 10    & 100   & 1000    \\ \midrule
Baseline                & 38.65 & 62.16 & 63.90*  \\
TC - Transformer Layer  & -0.70 & -0.03 & 0.10*   \\
TC - Feed-Forward Layer & 0.41 & 1.37 & -0.24* \\ \bottomrule
\end{tabular}

\caption{\label{tab:re_tc} NER results on join-training and our proposed method with two different model architectures as the transfer component placed after the embedding layer. TC denotes transfer component. }
\end{wraptable} 
